Communication Efficient Distributed Learning with Censored, Quantized, and Generalized Group ADMM

In this paper, we propose a communication-efficiently decentralized machine learning framework that solves a consensus optimization problem defined over a network of inter-connected workers. The proposed algorithm, Censored and Quantized Generalized GADMM (CQ-GGADMM), leverages the worker grouping and decentralized learning ideas of Group Alternating Direction Method of Multipliers (GADMM), and pushes the frontier in communication efficiency by extending its applicability to generalized network topologies, while incorporating link censoring for negligible updates after quantization. We theoretically prove that CQ-GGADMM achieves the linear convergence rate when the local objective functions are strongly convex under some mild assumptions. Numerical simulations corroborate that CQ-GGADMM exhibits higher communication efficiency in terms of the number of communication rounds and transmit energy consumption without compromising the accuracy and convergence speed, compared to the censored decentralized ADMM, and the worker grouping method of GADMM.

==> Notations.tex <==
\section{Notations}\label{Notations}
In this section, we introduce the notations and main assumptions that will be used throughout the paper.
\subsection{Notations}
\subsection{Assumptions}
\noindent We make the following assumptions required for the convergence proofs.\\
\textbf{Assumption 1.} The communication graph $\mathcal{G}$ is bipartite and connected.\\
\textbf{Assumption 2.} The local cost functions $f_n$ are closed, proper, and convex. \\
Note that this assumption ensures that the problem \textbf{(P2)} has a unique optimal solution, denoted by $\bm{\theta}^\star$.\\
\textbf{Assumption 3.} The unaugmented Lagrangian $\mathcal{L}_0$ has a saddle point.\\
\textbf{Assumption 4.} The local cost functions $f_n$ are strongly convex with parameter $\mu_n > 0$, i.e.
\begin{align}
\|\nabla f_n(\bm{x}) - \nabla f_n(\bm{y}) \| \geq \mu_n \|\bm{x}-\bm{y}\|^2, \forall \bm{x}, \bm{y} \in \mathbb{R}^d.
\end{align} 
Under this assumption, the function $f$ is strongly convex with parameter $\mu = \underset{1 \leq n \leq N}{\min}~\mu_n$.\\
\textbf{Assumption 5.} The local cost functions $f_n$ have $L_n$-Lipschitz continuous gradient ($L_n > 0$), i.e.
\begin{align}
\|\nabla f_n(\bm{x}) - \nabla f_n(\bm{y}) \| \leq L_n \|\bm{x}-\bm{y}\|, \forall \bm{x}, \bm{y} \in \mathbb{R}^d.
\end{align} 
Note that we can easily show that, in this case, $f$ has $L$-Lipschitz continuous gradient with $L = \underset{1 \leq n \leq N}{\min}~L_n$.
\textcolor{red}{try to see if assumption 2 and 3 can be somehow loosened}



==> quantization.tex <==
\linespread{1.33}
\section{Censored quantized GGADMM (C-QGGADMM)}
\label{qcgadmm}
C-GGADMM algorithm shows improvement in terms of the communication overhead over GGADMM algorithm, but still it needs to receives the full precission information $\boldsymbol{\theta}$'s from the neighbors at each worker $n$ to update the local model. This creates a communication bottleneck; especially when the dimensions $d$ of $\boldsymbol{\theta}$ is large. We address this issue using stochastic quantization in which we use the quantized version of the information $\hat{\boldsymbol{\theta}}_{m} \forall m \in {\cal N}_n$ to update the primal and dual variables at each worker $n$.   





%\subsection{Stochastic Quantization} \label{stochastic_quantixation}

We follow the same stochastic quantization scheme described in \cite{} where each worker quantizes the difference between its current model and its previously quantized model before transmission ({$\boldsymbol{\theta}_n^k-\boldsymbol{\hat\theta}_n^{k-1}$\nm}) as {$\boldsymbol{\theta}_n^k-\boldsymbol{\hat\theta}_n^{k-1} = Q_n(\boldsymbol{\theta}_n^k, \boldsymbol{\hat\theta}_n^{k-1})$\nm. The function {$Q_n(\cdot)$\nm} is a stochastic quantization operator that depends on the quantization probability $p_{n,i}^k$ for each model vector's dimension $i\in\{1,2,\cdots,d\}$, and on $b_n^k$ bits used for representing each model vector dimension. 

The $i$-th dimensional element {$[\boldsymbol{\hat\theta}_n^{k-1}]_i$\nm} of the previously quantized model vector is centered at the quantization range {$2 R_n^k$\nm} that is equally divided into $2^{b_n^k}-1$\nm~quantization levels, yielding the quantization step size $\Delta_n^k=2 R_n^k/(2^{b_n^k}-1)$\nm. In this coordinate, the difference between the $i$-th dimensional element {$[\boldsymbol{\theta}_n^k]_i$\nm} of the current model vector and {$[\boldsymbol{\hat\theta}_n^{k-1}]_i$\nm} is
\begin{align}\label{quantization}
[c_n(\boldsymbol\theta_n^k)]_i\!=\! \frac{1}{\Delta_n^k} \left([\boldsymbol\theta_n^k]_i-[\boldsymbol{\hat\theta}_n^{k-1}]_i\!+\!R_n^k\right)\!,
\end{align}
where adding $R_n^k$\nm~ensures the non-negativity of the quantized value. Then, {$[c_n(\boldsymbol\theta_n^k)]_i$\nm} is mapped to:
\begin{align}
[q_n(\boldsymbol\theta_n^k)]_i =\begin{cases}
\left\lceil [c_n(\boldsymbol\theta_n^k)]_i\!\right\rceil & \text{with probability $p_{n,i}^k$}\\[2pt]
\left\lfloor [c_n(\boldsymbol\theta_n^k)]_i\!\right\rfloor & \text{with probability $1-p_{n,i}^k$} \label{Eq:quant}
\end{cases}
\end{align}\nm
where $\lceil\cdot \rceil$ and $\lfloor\cdot \rfloor$ are ceiling and floor functions, respectively. 

%{\tblue{Let us denote the quantization error for the scheme in \eqref{Eq:quant} is denoted by $\boldsymbol{\epsilon}_{n,i}^k= [c_n(\boldsymbol\theta_n^k)]_i \!-\! \lfloor[c_n(\boldsymbol\theta_n^k)]_i \!\rfloor\!- [q_n(\boldsymbol\theta_n^k)]_i \!-\! \lfloor[c_n(\boldsymbol\theta_n^k)]_i \!\rfloor\!$. 

Next,  the probability $p_{n,i}^k$ in \eqref{Eq:quant} is selected such that the expected quantization error is $\mathbb{E}\left[\boldsymbol{\epsilon}_{n,i}^k\right]$ is zero \ie $p_{n,i}^k$ should satisfy: %}}  
%\E{\left[\boldsymbol{\epsilon}_{n,i}^k\right]}=
\begin{align}\label{mean_zero}
 p_{n,i}^k\!\left(\! [c_n(\boldsymbol\theta_n^k)]_i-\lceil[c_n(\boldsymbol\theta_n^k)]_i \!\rceil\!\! \right)\!+\!(1\!-\!p_{n,i}^k) \! \left( [c_n(\boldsymbol\theta_n^k)]_i -\! \lfloor[c_n(\boldsymbol\theta_n^k)]_i \!\rfloor\! \!\right)\!=\!0, 
\end{align}
Solving \eqref{mean_zero} for $p_{n,i}^k$, we obtain 
\vspace{-5pt}\begin{align}
p_{n,i}^k = \left(\! [c_n(\boldsymbol\theta_n^k)]_i-\lfloor[c_n(\boldsymbol\theta_n^k)]_i \!\rfloor\! \right)\label{Eq:Optp}%/\Delta_n^k 
\end{align}
%where the denominator follows from $\Delta_n^k = \lceil[c_n(\boldsymbol\theta_n^k)]_i \!\rceil - \lfloor[c_n(\boldsymbol\theta_n^k)]_i \!\rfloor$\nm.

The $p_{n,i}^k$ selection in \eqref{Eq:Optp} ensures that the quantization in \eqref{Eq:quant} is unbiased and the  quantization error variance $\mathbb{E}\left[\left(\boldsymbol{\epsilon}_{n,i}^k\right)^2\right]$ is equal to $({\Delta_n^k})^2/4$. This implies that $\mathbb{E}\left[\norm{\boldsymbol{\epsilon}_{n}^k}^2\right]= d({\Delta_n^k})^2/4$. 


In addition to the above condition, the convergence of C-QGGADMM requires non-increasing quantization step sizes over iterations, \ie $\Delta_n^k \leq \Delta_n^{k-1}$ for all $k$. To satisfy this condition, $b_n^k$ is chosen as
\begin{align}
b_n^k \geq \left\lceil \log_2\left(1 + (2^{b_n^{k-1}}-1)R_n^k/R_n^{k-1} \right) \right\rceil. \label{Eq:Optb}
\end{align}\nm
Given $p_{n,i}^k$ in \eqref{Eq:Optp} and $b_n^k$ in \eqref{Eq:Optb}, the convergence of C-QGADMM is provided in Sec.\ref{sec:convergence}. %We remark that in the numerical simulations (Sec.\ref{sec:sim}), we observe that $R_n^k$ decreases over iterations, and thus $\Delta_n^k \leq \Delta_n^{k-1}$\nm~holds even when $b_n^k$ is fixed.


With the aforementioned stochastic quantization procedure, $b_n^k$\nm, $R_n^k$\nm, and $q_n(\boldsymbol{\theta}_n^k)$ suffice to represent $\boldsymbol{\hat\theta}_n^k$, where
\begin{align}
q_n(\boldsymbol{\theta}_n^k)=( [q_n(\boldsymbol{\theta}_n^k)]_1,[q_n(\boldsymbol{\theta}_n^k)]_2,\cdots,[q_n(\boldsymbol{\theta}_n^k)]_d )^\intercal,
\end{align}
\noindent which are transmitted to neighbors. After receiving these values, $\boldsymbol{\hat\theta}_n^k$\nm~can be reconstructed as follows:
{\begin{align}
\hat{\boldsymbol\theta}_n^k = \boldsymbol{\hat\theta}_n^{k-1}+ \Delta_n^k q_n(\boldsymbol\theta_n^k)-R_n^k\mathbf{1}.
 \label{recoverEq}
 \end{align}\normalsize} 
\noindent Consequently, when the full arithmetic precision uses $32$bit, every transmission payload size of C-QGGADMM is $b_n^k d + (b_R + b_b)$ bits, where $b_R\leq 32$ and $b_b\leq 32$ are the required bits to represent $R_n^k$ and $b_n^k$, respectively. Compared to GGADMM whose payload size is $32d$ bits, Q-GADMM can achieve a huge reduction in communication overhead, particularly for large models, \ie large $d$.






